Image Watermarking With Memory Across Reissuance

Publishers often revise and reissue images, yet valid watermarks may persist on superseded releases or unapproved edits. Even a current release can contain regions last authorized at different revisions. We introduce and formalize reissuable provenance: determining an image's current, superseded, or unissued status and recovering each region's last authorized revision (its generation), with abstention when evidence is insufficient. Generational Stratigraphy Fields (GSF) combine watermark evidence with an authenticated live reference to the current release, enabling replacement or retirement without rewriting circulated copies. Each reissue freshly embeds new generation labels in approved regions and inherited labels elsewhere, preserving history without requiring old watermarks to survive successive edits. Our complete-output reissuance evaluation follows 480 histories through four releases, retaining each AI editor's entire output. GSF achieves 99.67% accuracy in classifying issued images as current or superseded and 94.09% recall of unissued edits. After three reissues, one generation map provides time and location: it recovers regional labels with 93.13% median accuracy and localizes the latest approved revision with 92.86% IoU. Regional labels remain readable under tested delivery transformations that impair issued-state recognition. Watermarks can thus express who issued an image, which release is authoritative now, and when each region was last authorized.

==> Ablations_and_Analysis.tex <==
\section{Ablations and Analysis}
\label{sec:ablations}

Three controlled comparisons identify what closes the lifecycle, what carries
the reader gain, and why spatial inference remains necessary under alternative
two-bit encodings.  We then test the fixed-slot rate--resolution prediction
derived in Section~\ref{sec:writer}.

\subsection{Which Evidence Closes the Lifecycle?}
\label{sec:ablation-lifecycle-evidence}

Registered-issue matching recognizes issued images but leaves most unissued
transitions unresolved.  Table~\ref{tab:lifecycle-evidence} adds evidence
cumulatively under the same frozen query schedule.  Carrier disruption raises
\textsc{Open} recall from 14.29\% to 88.65\%; adding lineage-conditioned issue
evidence and head-relative interpretation reaches 94.09\% while reducing false
issue acceptance.

\begin{table}[!htbp]
\caption{Cumulative lifecycle-evidence ablation (\%).  The oracle is a
diagnostic upper bound on the final unissued and earlier-issue subset
($2\times480$), not a fourth verifier operating point.}
\label{tab:lifecycle-evidence}
\centering
\small
\begin{tabular}{@{}lrrr@{}}
\toprule
Evidence used & Reg. acc. & \textsc{Open} recall & Issue FAR \\
\midrule
Registered-issue match only       & 99.88 & 14.29 & 4.92 \\
$+$ carrier-disruption evidence   & 99.88 & 88.65 & 4.92 \\
Full GSF decision                 & 99.67 & \textbf{94.09} & \textbf{2.24} \\
\midrule
Oracle upper bound (subset)       & -- & 98.23 & -- \\
\bottomrule
\end{tabular}
\end{table}

Full GSF retains 99.67\% registered-state accuracy while raising
\textsc{Open} recall from 14.29\% to 94.09\% and reducing false issue
acceptance from 4.92\% to 2.24\%.  Disruption opens the transition; lineage and
issue evidence determine whether an issued state still matches; and the live
head interprets that match as \textsc{Current} or \textsc{Superseded}.
Reissuance then closes the transition with a new registered issue.  Per-query
counts appear in Appendix~\ref{app:lifecycle-results}.

\subsection{Recalibration and Soft Spatial Coupling Carry the Reader Gain}
\label{sec:ablation-reader}

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth]{./fig/ablation_analysis.png}
\caption{Mechanisms behind spatial history recovery.  \textbf{(a)} Predicted
and observed ambiguity rise with depth; independent cell-wise accuracy falls,
while spatial recovery remains stable.  Each point summarizes 480 successors.
\textbf{(b)} Reader-mechanism attribution on the 480-root transfer set; the
dashed line is a hard spatial partition.  \textbf{(c)} Unique-anchor yield
under a fixed 320-slot budget.  Curves are
Eq.~\eqref{eq:fixed-slot-anchor-count}; hollow markers are measurements at the
three evaluated depths.}
\label{fig:ablation-summary}
\end{figure}

Figure~\ref{fig:ablation-summary} connects the reader's outcome to its cause.
At depths one, two, and three, the predicted ambiguous-cell fractions are
25.00\%, 43.75\%, and 57.81\%; the observed fractions are 24.38\%, 43.75\%,
and 58.13\%.  The close agreement shows that the loss of local identifiability
is the expected consequence of constant-rate history encoding.  Panel (a)
then shows the resulting separation: independent readout deteriorates with
depth, whereas spatial recovery remains stable.

Panel (b) identifies what carries that recovery.  Raw candidate likelihoods
obtain 36.97\% aggregate accuracy; shared pointwise recalibration raises this
to 67.48\%, and soft multiscale spatial coupling reaches 87.83\%.  A hard
partition reaches 80.78\%, whereas recurrence, content features, and auxiliary
state heads remain within 87.7--88.1\% without stable transfer improvement.
The gain is therefore carried by making temporal anchors reliable and
propagating them without an early hard partition.  Complete controls appear in
Appendix~\ref{app:spatial-reader-details}.

\FloatBarrier
\subsection{Spatial Inference Remains Necessary Beyond Code Collisions}
\label{sec:ablation-same-rate}

We hold the formal roots, committed revision fields, and 320 physical slots
fixed while changing the code assignment; learned readers are retrained under
the same frozen data rules.  On intact issued fields, the cell-pooled keyed
collision fractions at depths
one, two, and three are 0.2487, 0.4363, and 0.5781, each within 0.0013 of
$1-(3/4)^d$.  Within the present four-label window, a position-invariant direct
two-bit label code is injective and nearly eliminates this issued-cell
ambiguity.  This is a useful counterfactual: it removes the collision mechanism
without increasing the local rate.

Editing exposes the remaining information limit.  On cells whose decoded
two-bit observation has flipped away from the issued code, both keyed and
direct-code local decisions have exactly zero correct recovery.  Nonzero
recovery must therefore use evidence outside that cell: surviving temporal
anchors and spatial coherence.  Spatial inference remains necessary even when
issued-cell code collisions are removed.

A position-invariant direct two-bit label code is injective only within four
labels, whereas position-dependent keyed fingerprints remain queryable over
variable finite candidate sets at the cost quantified by
Eq.~\eqref{eq:collision-law}.  Because the carrier is jointly optimized with
its code and synchronization rule, alternative assignments are evaluated under
a deliberately baseline-favorable slot-level counterfactual; physical recoding
is quantified separately in Appendix~\ref{app:same-rate-counterfactual}.

\subsection{Two Bits Balance Anchors and Spatial Resolution at the Evaluated
Depths}
\label{sec:ablation-bitwidth}

Equations~\eqref{eq:fixed-slot-anchor-count}--\eqref{eq:normalized-maximin}
predict the code-width tradeoff before learning.  Suppressing only the finite
grouping remainder, two bits have worst relative efficiency $3/4$ over
$D=\{1,2,3\}$.  One bit falls at $d=3$ to
$192/343\approx0.560$, whereas every $b\geq3$ is already bounded by its
$d=1$ term,
\begin{equation}
  \frac{2(1-2^{-b})}{b}\leq\frac{7}{12}<\frac{3}{4}.
  \label{eq:ablation-maximin-bound}
\end{equation}
Thus $b=2$ is the unique normalized-maximin allocation under a fixed slot
budget, keyed-iid fingerprints, and the declared depth range.  The result is
depth-qualified rather than universal: relative to the immediately narrower
code, the second, third, fourth, and eighth bits first increase total anchor
count at $d\geq2,3,5,$ and $34$, respectively.  Deeper histories therefore
gradually favor wider fingerprints.

Our carrier has $S_{\mathrm{slot}}=320$, so two-bit grouping yields 160 logical
regions.  The largest grouping remainder over the evaluated widths is
$2/320=0.625\%$ and does not change their ordering.  Figure~\ref{fig:ablation-summary}c
confirms the prediction empirically.  At depth three, locally unique readout is
0.127, 0.423, 0.673, 0.822, and 0.989 for $b=1,2,3,4,8$, versus closed-form
values 0.125, 0.422, 0.670, 0.824, and 0.988; every deviation is at most 0.003.

The learned readout obeys the same separation.  Regrouping keyed slots changes
collision geometry but not their marginal evidence law: independently trained
two- and eight-bit readers differ by 0.006 in pooled accuracy over 480 roots.
At the narrow end, one keyed bit leaves 87.5\% of regions ambiguous at depth
three, while a direct one-bit code aliases once three labels are registered.
At the wide end, eight bits leave only 40 logical regions, and 58.05\% of
deepest-field groups cross generation boundaries.  In fully damaged windows,
one- and two-bit local recovery is exactly zero; the small residual at coarser
widths comes from boundary-crossing groups rather than recovered evidence.
Thus two bits are not a universal optimum, but the measured balance of anchor
coverage and spatial resolution over the evaluated lifecycle depths.  The
proof, full width ladder, grouping controls, and deeper-history sensitivity are
in Appendix~\ref{app:bitwidth-ladder}.

Together, complementary lifecycle evidence closes issue-level transitions,
while temporal anchors, evidence recalibration, and soft spatial inference
preserve authorized history at the regional level.
\FloatBarrier


==> main_old.tex <==
% \documentclass{article}

% % Official ICLR 2027 submission style.
% \usepackage{iclr2027_conference,times}

% % Standard content packages used by the paper body.  They do not modify the
% % ICLR page geometry or style parameters.
% \usepackage{amsmath,amssymb}
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage{flafter}
% \usepackage[below]{placeins}
% \usepackage{xcolor}
% \usepackage{hyperref}
% \usepackage{url}

% % LaTeX provides \newtheorem; the official style does not predefine this name.

% \newtheorem{proposition}{Proposition}

% % Float and caption separations.  The ICLR style leaves these at LaTeX's
% % article defaults (12/20/12 pt, 10 pt above a caption); the values below
% % keep the style's font, margins, and 11-pt leading untouched.
% \setlength{\textfloatsep}{6pt plus 2pt minus 2pt}
% \setlength{\floatsep}{6pt plus 2pt minus 2pt}
% \setlength{\intextsep}{6pt plus 2pt minus 2pt}
% \setlength{\abovecaptionskip}{4pt}
% \setlength{\belowcaptionskip}{0pt}
% % A table title sits at the top of its float, so the float separation already
% % counts toward the space before it; together they make one line (11 pt).
% \AddToHook{env/table/begin}{\setlength{\abovecaptionskip}{5pt}}
% \AddToHook{env/table*/begin}{\setlength{\abovecaptionskip}{5pt}}

% % Revision of the discussion period: text added or rewritten in the revision is
% % set in this color (for the camera-ready version, set it to black).  Tables
% % added in the revision carry the numbers they have in the rebuttal (Table R1,
% % R2, ...), so that the submission's tables keep their numbers; \revfit scales
% % such a table down only if it is wider than the text.
% \definecolor{revcolor}{RGB}{0,70,180}
% \DeclareRobustCommand{\rev}[1]{{\color{revcolor}#1}}
% \newenvironment{revblock}{\color{revcolor}}{}
% \newcommand{\revtable}[1]{\color{revcolor}\addtocounter{table}{-1}%
%   \renewcommand{\thetable}{#1}\def\theHtable{#1}}
% \newcommand{\revfit}[1]{\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{#1}}

% \title{Image Watermarking with Memory\\across Reissuance}

% % Keep authors anonymous for review.  Do not enable \iclrfinalcopy here.
% \author{Anonymous authors}

% \begin{document}

% \maketitle

% \input{abstract}
% \input{introduction}
% \input{related_work}
% \input{problem_method}
% \input{result}

% \input{Conclusion}
% \input{statements}

% \bibliography{references}
% \bibliographystyle{iclr2027_conference}

% \clearpage
% \appendix
% % Appendix float policy (main text unaffected): floats sit with their text;
% % a float page is made only when nearly full, and stacks from the top.
% \renewcommand{\floatpagefraction}{0.85}
% \renewcommand{\topfraction}{0.9}
% \renewcommand{\bottomfraction}{0.5}
% \renewcommand{\textfraction}{0.1}
% \setcounter{topnumber}{3}
% \setcounter{bottomnumber}{2}
% \setcounter{totalnumber}{4}
% \makeatletter
% \setlength{\@fptop}{0pt}
% \setlength{\@fpsep}{8pt plus 2pt}
% \setlength{\@fpbot}{0pt plus 1fil}
% \makeatother
% \input{./appendix/appendix_a_semantics_reproducibility}
% \input{./appendix/appendix_b_implementation_training}
% \input{./appendix/appendix_c_evaluation_ground_truth}
% \input{./appendix/appendix_d_lifecycle_results}
% \input{./appendix/appendix_e_rendition_robustness}
% \input{./appendix/appendix_f_spatial_reader}
% \input{./appendix/appendix_g_generation_maps}
% \input{./appendix/appendix_h_resolution_canonicalization}
% \input{./appendix/appendix_i_complete_output_controls}
% \input{./appendix/appendix_j_statistics_scope}
% \input{./appendix/appendix_k_same_rate_counterfactual}
% \input{./appendix/appendix_l_bitwidth_ladder}
% \input{./appendix/appendix_m_cross_method_comparison}
% \input{./appendix/appendix_n_negative_queries}
% \input{./appendix/appendix_o_mark_preserving_edits}
% \input{./appendix/appendix_p_active_attacks}
% \end{document}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

